Example Exact Solutions of the Time-independent Gross-Pitaevskii and Schr\"odinger Equations

A prescription is given to obtain some exact results for certain external potentials $V\left({\vec r}\right)$ of the time-independent Gross-Pitaevskii and Schr\"odinger equations. The study motivation is the ability to program $V\left({\vec r}\right)$ experimentally in Bose-Einstein condensates. Rather than derive wavefunctions that are solutions for a given $V\left({\vec r}\right)$, we ask which $V\left({\vec r}\right)$ will have a given pdf (probability density function) $P\left({\vec r}\right)$. Several examples in 1D and 2D are presented for well-known pdfs and for the hydrogen atom in momentum space.

==> DUMMY-cut-paste.tex <==

\clearpage
\vfill\eject
\noindent{\bf XXX FIX BELOW XXX}

\begin{figure}[htp]
    \centering
    \includegraphics[width=8.6 cm]{P_n00-Hatom.png}
    \caption{XXX
    }
    \label{Fig:XXX1}
\end{figure}
%\FloatBarrier


\begin{figure}[htp]
    \centering
    \includegraphics[width=17.0 cm]{V-both_2-Hatom.PNG}
    \caption{XXX
    }
    \label{Fig:XXX3}
\end{figure}
%\FloatBarrier

Almost a century ago, Bose \cite{bose1924plancks} and Einstein \cite{einstein2005quantentheorie} introduced what is sometimes 
called the fifth state of matter, the Bose Einstein Condensate (BEC). It was not until 1995 that the first BEC was created
in a laboratory by using gases of ultra-cold atoms of Rb$^{87}$ and Na$^{23}$.  The 2001 Nobel Prize in Physics was awarded 
to these researchers for the experimental demonstration of 
a BEC \cite{XXX}.  The developing field of atomtronics
attempts to use a BEC condensate for quantum sensing, 
quantum computing, and quantum information science \cite{XXX}.
The project reported on here is motivated by the recent 
introduction of a stand-alone device by the company ColdQuanta 
\cite{XXX} where a BEC can be created and the BEC is in an 
external potential $V\left({\vec r}\right)$ which can be \lq painted' 
to have particular values in 2D (2 dimensions).  

The underlying equation for a BEC condensate 
\cite{ERDOS2007} has been rigorously shown, with reasonable 
assumptions, to be the Gross-Pitaevskii equation 
(GPeq), which is 
sometimes call the non-linear Schr{\"o}dinger equation. 
If the gas used for the BEC has $N$ atoms of mass $m$ and 
a scattering length $a_s$, the 
nonlinear term in the GPeq is $g=4\pi\hbar^2 a_s/m$ 
where $\hbar$ is Plank's constant divided by $2\pi$.  
The time-independent GPeq is
\begin{equation}
\label{Eq:GPeq:OLD}
\mu \psi\left({\vec r}\right) = 
\left(
-\frac{\hbar^2}{2m} \nabla^2 + V\left({\vec r}\right) 
+ g N \left|\psi\left({\vec r}\right)\right|^2 
\right) \psi\left({\vec r}\right)
\end{equation}
with $\mu$ the chemical potential.  
Here $\psi\left({\vec r}\right)$ is the wavefunction 
of the groundstate of the BEC.  

If $g=0$ and renaming $\mu$ to be the energy $E$ gives 
the normal time-independent Schr{\"o}dinger equation 
(TISE), namely
\begin{equation}
\label{Eq:TISE:OLD}
-\frac{\hbar^2}{2m}\nabla^2\psi\left({\vec r}\right) 
+ 
\left[ V\left({\vec r}\right)-E
\right]\psi\left({\vec r}\right) 
\> = \> 0
\>.
\end{equation}

\clearpage
\vfill\eject

and Li$^7$ [3,4]. Since past two decades, BEC is widely used in the fields of condensed matter physics and quantum computing [5]. Gross [6] and Pitaevskii [7] developed the equation to explain BEC which is analogus to Nonlinear Schr{\"o}dinger's Equation(NLSE). Quantum Mechanical Systems(QMS) provides an output in terms of probabilities which can be used to infer the properties of the QMS. Pioneering work to obtain such probabilities for QMS was done by [8] using Schr{\"o}dinger wave equations. To solve Schr{\"o}dinger wave equations, so far researchers explored the traditional approach by applying potentials to the QMS to get the distributions

\clearpage
\vfill\eject

{\bf DUMMY: \cite{Novotny2014}}

\begin{equation}
\label{Eq:pdfQu:01}
\begin{array}{c}
XXX \\
XXX \\
\end{array}
\end{equation}

\clearpage
\vfill\eject
